Turing degrees of multidimensional SFTs

In this paper we are interested in computability aspects of subshifts and in particular Turing degrees of 2-dimensional SFTs (i.e. tilings). To be more precise, we prove that given any \pizu subset $P$ of $\{0,1\}^\NN$ there is a SFT $X$ such that $P\times\ZZ^2$ is recursively homeomorphic to $X\setminus U$ where $U$ is a computable set of points. As a consequence, if $P$ contains a recursive member, $P$ and $X$ have the exact same set of Turing degrees. On the other hand, we prove that if $X$ contains only non-recursive members, some of its members always have different but comparable degrees. This gives a fairly complete study of Turing degrees of SFTs.

==> figures/tmtiling2.tex <==

\input figures/texcommands
\scalebox{0.4}{
\begin{tikzpicture}[scale=0.25]
\clip[draw,decorate,decoration={random steps,segment length=3pt,amplitude=1pt}]
(-3.5,-1.5) rectangle +(90,95);

\fill[bGunQuartBas] (5,1.8) rectangle (120,-4);\fill[unQuartBas] (5,1.8) rectangle (120,-4);

\fill[carreDownLeft] (7,3) -- ++ (3,3) -- ++ (0,-3) -- cycle;
\fill[carreDownLeft] (15,3) -- ++ (3,3) -- ++ (0,-3) -- cycle;
\fill[carreDownLeft] (27,3) -- ++ (3,3) -- ++ (0,-3) -- cycle;
\fill[carreDownLeft] (43,3) -- ++ (3,3) -- ++ (0,-3) -- cycle;
\fill[carreDownLeft] (63,3) -- ++ (3,3) -- ++ (0,-3) -- cycle;

\fill[carreDownLeft] (14,14) -- ++ (8,8) -- ++ (0,-8) -- cycle;
\fill[carreDownLeft] (26,18) -- ++ (8,8) -- ++ (0,-8) -- cycle;
\fill[carreDownLeft] (42,22) -- ++ (8,8) -- ++ (0,-8) -- cycle;
\fill[carreDownLeft] (62,26) -- ++ (8,8) -- ++ (0,-8) -- cycle;

\fill[carreDownLeft] (26,34) -- ++ (12,12) -- ++ (0,-12) -- cycle;
\fill[carreDownLeft] (42,42) -- ++ (12,12) -- ++ (0,-12) -- cycle;
\fill[carreDownLeft] (62,50) -- ++ (12,12) -- ++ (0,-12) -- cycle;

\fill[carreDownLeft] (42,62) -- ++ (16,16) -- ++ (0,-16) -- cycle;
\fill[carreDownLeft] (62,74) -- ++ (16,16) -- ++ (0,-16) -- cycle;

\fill[bGcarreDownRight] (6,2)  -- ++(1,1) -- ++ (3,0) -- ++ (0,3) -- ++ (4,4)   -- ++(0,-8) -- cycle;
\fill[bGcarreDownRight] (14,2) -- ++(1,1) -- ++ (3,0) -- ++ (0,3) -- ++ (8,8)   -- ++(0,-12) -- cycle;
\fill[bGcarreDownRight] (26,2) -- ++(1,1) -- ++ (3,0) -- ++ (0,3) -- ++ (12,12) -- ++(0,-16) -- cycle;
\fill[bGcarreDownRight] (42,2) -- ++(1,1) -- ++ (3,0) -- ++ (0,3) -- ++ (16,16) -- ++(0,-20) -- cycle;
\fill[bGcarreDownRight] (62,2) -- ++(1,1) -- ++ (3,0) -- ++ (0,3) -- ++ (20,20) -- ++(0,-24) -- cycle;
\fill[bGcarreDownRight] (86,2) -- ++(1,1) -- ++ (3,0) -- ++ (0,3) -- ++ (24,24) -- ++(0,-28) -- cycle;


\fill[bGcarreDownRight] (18,14) -- ++ (0,1) -- ++ (4,0) -- ++ (0,7) -- ++ (4,4)   -- ++(0,-12) -- cycle;
\fill[bGcarreDownRight] (30,18) -- ++ (0,1) -- ++ (4,0) -- ++ (0,7) -- ++ (8,8)   -- ++(0,-16) -- cycle;
\fill[bGcarreDownRight] (46,22) -- ++ (0,1) -- ++ (4,0) -- ++ (0,7) -- ++ (12,12)   -- ++(0,-20) -- cycle;
\fill[bGcarreDownRight] (66,26) -- ++ (0,1) -- ++ (4,0) -- ++ (0,7) -- ++ (16,16)   -- ++(0,-24) -- cycle;

\fill[bGcarreDownRight] (34,34) -- ++ (0,1) -- ++ (4,0) -- ++ (0,11) -- ++ (4,4)   -- ++(0,-16) -- cycle;
\fill[bGcarreDownRight] (50,42) -- ++ (0,1) -- ++ (4,0) -- ++ (0,11) -- ++ (8,8)   -- ++(0,-20) -- cycle;
\fill[bGcarreDownRight] (70,50) -- ++ (0,1) -- ++ (4,0) -- ++ (0,11) -- ++ (12,12)   -- ++(0,-24) -- cycle;

\fill[bGcarreDownRight] (54,62) -- ++ (0,1) -- ++ (4,0) -- ++ (0,15) -- ++ (4,4)   -- ++(0,-20) -- cycle;
\fill[bGcarreDownRight] (74,74) -- ++ (0,1) -- ++ (4,0) -- ++ (0,15) -- ++ (8,8)   -- ++(0,-24) -- cycle;

\fill[carreDownRight] (6,2)  -- ++(1,1) -- ++ (3,0) -- ++ (0,3) -- ++ (4,4)   -- ++(0,-8) -- cycle;
\fill[carreDownRight] (14,2) -- ++(1,1) -- ++ (3,0) -- ++ (0,3) -- ++ (8,8)   -- ++(0,-12) -- cycle;
\fill[carreDownRight] (26,2) -- ++(1,1) -- ++ (3,0) -- ++ (0,3) -- ++ (12,12) -- ++(0,-16) -- cycle;
\fill[carreDownRight] (42,2) -- ++(1,1) -- ++ (3,0) -- ++ (0,3) -- ++ (16,16) -- ++(0,-20) -- cycle;
\fill[carreDownRight] (62,2) -- ++(1,1) -- ++ (3,0) -- ++ (0,3) -- ++ (20,20) -- ++(0,-24) -- cycle;
\fill[carreDownRight] (86,2) -- ++(1,1) -- ++ (3,0) -- ++ (0,3) -- ++ (24,24) -- ++(0,-28) -- cycle;


\fill[carreDownRight] (18,14) -- ++ (0,1) -- ++ (4,0) -- ++ (0,7) -- ++ (4,4)   -- ++(0,-12) -- cycle;
\fill[carreDownRight] (30,18) -- ++ (0,1) -- ++ (4,0) -- ++ (0,7) -- ++ (8,8)   -- ++(0,-16) -- cycle;
\fill[carreDownRight] (46,22) -- ++ (0,1) -- ++ (4,0) -- ++ (0,7) -- ++ (12,12)   -- ++(0,-20) -- cycle;
\fill[carreDownRight] (66,26) -- ++ (0,1) -- ++ (4,0) -- ++ (0,7) -- ++ (16,16)   -- ++(0,-24) -- cycle;

\fill[carreDownRight] (34,34) -- ++ (0,1) -- ++ (4,0) -- ++ (0,11) -- ++ (4,4)   -- ++(0,-16) -- cycle;
\fill[carreDownRight] (50,42) -- ++ (0,1) -- ++ (4,0) -- ++ (0,11) -- ++ (8,8)   -- ++(0,-20) -- cycle;
\fill[carreDownRight] (70,50) -- ++ (0,1) -- ++ (4,0) -- ++ (0,11) -- ++ (12,12)   -- ++(0,-24) -- cycle;

\fill[carreDownRight] (54,62) -- ++ (0,1) -- ++ (4,0) -- ++ (0,15) -- ++ (4,4)   -- ++(0,-20) -- cycle;
\fill[carreDownRight] (74,74) -- ++ (0,1) -- ++ (4,0) -- ++ (0,15) -- ++ (8,8)   -- ++(0,-24) -- cycle;

\fill[carreUpLeft] (6.2,2.2) -- ++(3.8,3.8) -- ++(0,3.8) -- ++(-3.8,0) -- cycle;
\fill[carreUpLeft] (14.2,2.2) -- ++(3.8,3.8) -- ++(0,7.8) -- ++(-3.8,0) -- cycle;
\fill[carreUpLeft] (26.2,2.2) -- ++(3.8,3.8) -- ++(0,11.8) -- ++(-3.8,0) -- cycle;
\fill[carreUpLeft] (42.2,2.2) -- ++(3.8,3.8) -- ++(0,15.8) -- ++(-3.8,0) -- cycle;
\fill[carreUpLeft] (62.2,2.2) -- ++(3.8,3.8) -- ++(0,19.8) -- ++(-3.8,0) -- cycle;
\fill[carreUpLeft] (86.2,2.2) -- ++(3.8,3.8) -- ++(0,23.8) -- ++(-3.8,0) -- cycle;

\fill[carreUpLeft] (14.2,14.2) -- ++(7.8,7.8) -- ++(0,3.8) -- ++(-7.8,0) -- cycle;
\fill[carreUpLeft] (26.2,18.2) -- ++(7.8,7.8) -- ++(0,7.8) -- ++(-7.8,0) -- cycle;
\fill[carreUpLeft] (42.2,22.2) -- ++(7.8,7.8) -- ++(0,11.8) -- ++(-7.8,0) -- cycle;
\fill[carreUpLeft] (62.2,26.2) -- ++(7.8,7.8) -- ++(0,15.8) -- ++(-7.8,0) -- cycle;
\fill[carreUpLeft] (86.2,30.2) -- ++(7.8,7.8) -- ++(0,19.8) -- ++(-7.8,0) -- cycle;

\fill[carreUpLeft] (26.2,34.2) -- ++(11.8,11.8) -- ++(0,3.8) -- ++(-11.8,0) -- cycle;
\fill[carreUpLeft] (42.2,42.2) -- ++(11.8,11.8) -- ++(0,7.8) -- ++(-11.8,0) -- cycle;
\fill[carreUpLeft] (62.2,50.2) -- ++(11.8,11.8) -- ++(0,11.8) -- ++(-11.8,0) -- cycle;
\fill[carreUpLeft] (86.2,58.2) -- ++(11.8,11.8) -- ++(0,15.8) -- ++(-11.8,0) -- cycle;

\fill[carreUpLeft] (42.2,62.2) -- ++(15.8,15.8) -- ++(0,3.8) -- ++(-15.8,0) -- cycle;
\fill[carreUpLeft] (62.2,74.2) -- ++(15.8,15.8) -- ++(0,7.8) -- ++(-15.8,0) -- cycle;
\fill[carreUpLeft] (86.2,86.2) -- ++(15.8,15.8) -- ++(0,11.8) -- ++(-15.8,0) -- cycle;

\fill[bGcarreUpRight] (10,6) -- ++(4,4) -- ++(-4,0) -- cycle;
\fill[bGcarreUpRight] (22,22) -- ++(4,4) -- ++(-4,0) -- cycle;
\fill[bGcarreUpRight] (38,46) -- ++(4,4) -- ++(-4,0) -- cycle;
\fill[bGcarreUpRight] (58,78) -- ++(4,4) -- ++(-4,0) -- cycle;

\fill[bGcarreUpRight] (18,6) -- ++(8,8) -- ++(-8,0) -- cycle;
\fill[bGcarreUpRight] (34,26) -- ++(8,8) -- ++(-8,0) -- cycle;
\fill[bGcarreUpRight] (54,54) -- ++(8,8) -- ++(-8,0) -- cycle;
\fill[bGcarreUpRight] (78,90) -- ++(8,8) -- ++(-8,0) -- cycle;

\fill[bGcarreUpRight] (30,6) -- ++(12,12) -- ++(-12,0) -- cycle;
\fill[bGcarreUpRight] (50,30) -- ++(12,12) -- ++(-12,0) -- cycle;
\fill[bGcarreUpRight] (74,62) -- ++(12,12) -- ++(-12,0) -- cycle;

\fill[bGcarreUpRight] (46,6) -- ++(16,16) -- ++(-16,0) -- cycle;
\fill[bGcarreUpRight] (70,34) -- ++(16,16) -- ++(-16,0) -- cycle;

\fill[bGcarreUpRight] (66,6) -- ++(20,20) -- ++(-20,0) -- cycle;



\fill[carreUpRight] (10,6) -- ++(4,4) -- ++(-4,0) -- cycle;
\fill[carreUpRight] (22,22) -- ++(4,4) -- ++(-4,0) -- cycle;
\fill[carreUpRight] (38,46) -- ++(4,4) -- ++(-4,0) -- cycle;
\fill[carreUpRight] (58,78) -- ++(4,4) -- ++(-4,0) -- cycle;

\fill[carreUpRight] (18,6) -- ++(8,8) -- ++(-8,0) -- cycle;
\fill[carreUpRight] (34,26) -- ++(8,8) -- ++(-8,0) -- cycle;
\fill[carreUpRight] (54,54) -- ++(8,8) -- ++(-8,0) -- cycle;
\fill[carreUpRight] (78,90) -- ++(8,8) -- ++(-8,0) -- cycle;

\fill[carreUpRight] (30,6) -- ++(12,12) -- ++(-12,0) -- cycle;
\fill[carreUpRight] (50,30) -- ++(12,12) -- ++(-12,0) -- cycle;
\fill[carreUpRight] (74,62) -- ++(12,12) -- ++(-12,0) -- cycle;

\fill[carreUpRight] (46,6) -- ++(16,16) -- ++(-16,0) -- cycle;
\fill[carreUpRight] (70,34) -- ++(16,16) -- ++(-16,0) -- cycle;

\fill[carreUpRight] (66,6) -- ++(20,20) -- ++(-20,0) -- cycle;

\fill[carreBorder] (4.8,2) rectangle (5.2,-4);

\fill[carreBorder] (5.8,2.2) rectangle ++(.4,8);
\fill[carreBorder] (13.8,2.2) rectangle ++(.4,24);
\fill[carreBorder] (25.8,2.2) rectangle ++(.4,48);
\fill[carreBorder] (41.8,2.2) rectangle ++(.4,80);
\fill[carreBorder] (61.8,2.2) rectangle ++(.4,100);
\fill[carreBorder] (85.8,2.2) rectangle ++(.4,100);

\fill[carreBorder] (5.8,10.2) rectangle ++(8,-.4);
\fill[carreBorder] (13.8,14.2) rectangle ++(12,-.4);
\fill[carreBorder] (13.8,26.2) rectangle ++(12,-.4);
\fill[carreBorder] (25.8,18.2) rectangle ++(16,-.4);
\fill[carreBorder] (25.8,34.2) rectangle ++(16,-.4);
\fill[carreBorder] (25.8,50.2) rectangle ++(16,-.4);
\fill[carreBorder] (41.8,22.2) rectangle ++(20,-.4);
\fill[carreBorder] (41.8,42.2) rectangle ++(20,-.4);
\fill[carreBorder] (41.8,62.2) rectangle ++(20,-.4);
\fill[carreBorder] (41.8,82.2) rectangle ++(20,-.4);
\fill[carreBorder] (61.8,26.2) rectangle ++(24,-.4);
\fill[carreBorder] (61.8,50.2) rectangle ++(24,-.4);
\fill[carreBorder] (61.8,74.2) rectangle ++(24,-.4);
\fill[carreBorder] (61.8,98.2) rectangle ++(24,-.4);
\fill[carreBorder] (85.8,30.2) rectangle ++(28,-.4);
\fill[carreBorder] (85.8,58.2) rectangle ++(28,-.4);
\fill[carreBorder] (85.8,86.2) rectangle ++(28,-.4);
\fill[carreBorder] (4.8,1.8) rectangle ++(100,.4);

\fill[signalBas] (4.8,2.2) rectangle ++(.4,4) rectangle ++ (2,-0.4) rectangle ++ (-0.4,4.4) rectangle ++ (6,-.4);
\fill[signalBas] (12.8,2.2) rectangle ++(.4,8) rectangle ++ (2,-0.4) rectangle ++ (-0.4,4.4) rectangle ++ (10,-.4);
\fill[signalBas] (24.8,2.2) rectangle ++(.4,12) rectangle ++ (2,-0.4) rectangle ++ (-0.4,4.4) rectangle ++ (14,-.4);
\fill[signalBas] (40.8,2.2) rectangle ++(.4,16) rectangle ++ (2,-0.4) rectangle ++ (-0.4,4.4) rectangle ++ (18,-.4);
\fill[signalBas] (60.8,2.2) rectangle ++(.4,20) rectangle ++ (2,-0.4) rectangle ++ (-0.4,4.4) rectangle ++ (22,-.4);
\fill[signalBas] (84.8,2.2) rectangle ++(.4,24) rectangle ++ (2,-0.4) ;

\fill[signalCarres] (6.2,2.8) rectangle ++(4,0.4) rectangle ++(-0.4,8) rectangle ++ (4,-0.4);
\fill[signalCarres] (14.2,2.8) rectangle ++(4,0.4) rectangle ++(-0.4,12)  rectangle ++ (4.4,-0.4) rectangle ++(-0.4,12) rectangle ++ (4,+0.4);
\fill[signalCarres] (26.2,2.8) rectangle ++(4,0.4) rectangle ++(-0.4,16)  rectangle ++ (4.4,-0.4) rectangle ++(-0.4,16) 
rectangle ++ (4.4,+0.4) rectangle ++(-0.4,16) rectangle ++ (4,-0.4);
\fill[signalCarres] (42.2,2.8) rectangle ++(4,0.4) rectangle ++(-0.4,20)  rectangle ++ (4.4,-0.4) rectangle ++(-0.4,20)
rectangle ++ (4.4,+0.4) rectangle ++(-0.4,20) rectangle ++ (4.4,-0.4) rectangle ++ (-0.4,20) rectangle ++ (4,0.4);
\fill[signalCarres] (62.2,2.8) rectangle ++(4,0.4) rectangle ++(-0.4,24)  rectangle ++ (4.4,-0.4) rectangle ++(-0.4,24)
rectangle ++ (4.4,+0.4) rectangle ++(-0.4,24) rectangle ++ (4.4,-0.4) rectangle ++ (-0.4,24) rectangle ++ (4,0.4);
\fill[signalCarres] (86.2,2.8) rectangle ++(4,0.4);

\draw[scale=4] (-3,-4) grid +(120,120);

\end{tikzpicture}
}

